Combined Scheduling, Memory Allocation and Tensor Replacement for Minimizing Off-Chip Data Accesses of DNN Accelerators

Specialized hardware accelerators have been extensively used for Deep Neural Networks (DNNs) to provide power/performance benefits. These accelerators contain specialized hardware that supports DNN operators, and scratchpad memory for storing the tensor operands. Often, the size of the scratchpad is insufficient to store all the tensors needed for the computation, and additional data accesses are needed to move tensors back and forth from host memory during the computation with significant power/performance overhead. The volume of these additional data accesses depends on the operator schedule, and memory allocation (specific locations selected for the tensors in the scratchpad). We propose an optimization framework, named COSMA, for mapping DNNs to an accelerator that finds the optimal operator schedule, memory allocation and tensor replacement that minimizes the additional data accesses. COSMA provides an Integer Linear Programming (ILP) formulation to generate the optimal solution for mapping a DNN to the accelerator for a given scratchpad size. We demonstrate that, using an off-the-shelf ILP solver, COSMA obtains the optimal solution in seconds for a wide-range of state-of-the-art DNNs for different applications. Further, it out-performs existing methods by reducing on average 84% of the non-compulsory data accesses. We further propose a divide-and-conquer heuristic to scale up to certain complex DNNs generated by Neural Architecture Search, and this heuristic solution reduces on average 85% data accesses compared with other works.

==> discussion.tex <==
\section{Discussion}
% \subsection{Operator Granularity}
\name is flexible on the operator granularity. In this prototype, we focus on coarse-grain hardware accelerators, but \name can be adapted to support finer-grain operations
% \subsection{Limitation of \name}
\name is limited to DNNs with statically determined behaviors.
Also in the current divide-and-conquer technique to support complex models, we rely on expert's inputs to divide the models into smaller graphs. One promising way is to formulate the graph division problem and automate it.

==> floats/bg-table.tex <==
\begin{table}[ht]
\captionsetup{font=small}
\caption{\small Methodology Comparison}
\centering

\label{tab:bg-table}
\end{table}

==> floats/ilp-mem-alloc.tex <==
\begin{equation}
\small
\label{mem-alloc-c1}
\begin{aligned}
    &\forall t \in T, \forall a \in A, & &\:L_{a, t} \: + \: Size(a) \leq M_{B}
\end{aligned}
\end{equation}

\begin{equation}
\small
\label{mem-alloc-c2}\
\begin{aligned}
    \forall t \in T, \forall (a, b) \in A^{2}, \;\;
        u_{a,\: b,\: t} + d_{a,\: b,\: t} &\leq& &1 \\
        u_{a,\: b,\: t} + d_{a,\: b,\: t} &\geq& &res_{a,\: t} + res_{b,\: t} - 1 \\
        L_{a, t} + Size(a) - L_{b,\: t} &\leq& & M \times (1 - d_{a,\: b,\: t}) \\
        L_{b, t} + Size(b) - L_{a,\: t} & \leq& & M \times (1 - u_{a,\: b,\: t}) \\
        \text{where  } \; res_{a,\: t} &=& &C_{a,\: t} + P_{a,\: t} + R_{a,\: t} \\
        \text{and  } \; res_{b,\: t} &=& &C_{b,\: t} + P_{b,\: t} + R_{b,\: t}
\end{aligned}
\end{equation}

\begin{equation}
\small
\label{mem-alloc-c3}\
\begin{aligned}
    \forall t \in T, \forall a \in A, \;\;
        L_{a, \: t-1} - L_{a, \: t} & \leq & &M \times (1 - T_{a, \: t}) \\
        L_{a, \: t} - L_{a, \: t-1} & \leq & &M \times (1 - T_{a, \: t}) \\
        T_{a, \: t} & \geq & &(C_{a, \: t-1} + P_{a, \: t-1} + R_{a, \: t-1}) + P_{a, \: t} - 1 \\ 
        T_{a, \: t} & \leq & &(C_{a, \: t-1} + P_{a, \: t-1} + R_{a, \: t-1}) \\
        T_{a, \: t} & \leq & &P_{a, \: t}
\end{aligned}
\end{equation}

==> floats/ilp-sch.tex <==
% \small
% \begin{align}
% \label{sch-c-1}
% &\forall t \in T, \forall a \in A, & &\:C_{a, t} + P_{a, t} + S_{a, t} + R_{a, t} \leq 1\\
% \label{sch-c-2}
% &\forall t \in T, \forall a \in A, & &\:P_{a, t} \leq C_{a, t-1} + P_{a, t-1} + R_{a, t-1}\\
% \label{sch-c-3}
% &\forall t \in T, \forall a \in A, & &\:S_{a, t} \leq C_{a, t-1} + P_{a, t-1}\\
% \label{sch-c-4}
% &\forall t \in T, \forall a \in A, & &\:R_{a, t} \leq \textstyle\sum\limits_{\scriptscriptstyle k=0}^{\scriptscriptstyle t} S_{a, k}\\
% \label{sch-c-5}
% &\forall a \in A, & &\:\textstyle\sum\limits_{\scriptscriptstyle t \in T} C_{a, t} = 1 \\
% \label{sch-c-6}
% &\forall a \in A, & &\:\textstyle\sum\limits_{\scriptscriptstyle t \in T} S_{a, t} = 1 \\
% \label{sch-c-7}
% &\forall t \in T, \forall a \in A, & &\:\forall b \in in(a), \:C_{a, t} \leq P(b, t) + R(b, t)\\
% \label{sch-c-8}
% &\forall t \in T, \forall a \in A, & &\:\forall b \in sib(a), \:C(a, t) = C(b, t)\\
% \label{sch-c-9}
% &\forall t \in T, & &\:\textstyle\sum\limits_{\scriptscriptstyle a \in A} C_{a, t} = 1
% \end{align}
% \normalsize

\begin{subequations}
\label{eq:op-sch-constr}
\small
\begin{align}
    \label{sch-c-1}
&\forall t \in T, \forall a \in A, & &\:C_{a, t} + P_{a, t} + S_{a, t} + R_{a, t} \leq 1\\
\label{sch-c-2}
&\forall t \in T, \forall a \in A, & &\:P_{a, t} \leq C_{a, t-1} + P_{a, t-1} + R_{a, t-1}\\
\label{sch-c-3}
&\forall t \in T, \forall a \in A, & &\:S_{a, t} \leq C_{a, t-1} + P_{a, t-1}\\
\label{sch-c-4}
&\forall t \in T, \forall a \in A, & &\:R_{a, t} \leq \textstyle\sum\limits_{\scriptscriptstyle k=0}^{\scriptscriptstyle t} S_{a, k}\\
\label{sch-c-5}
&\forall a \in A, & &\:\textstyle\sum\limits_{\scriptscriptstyle t \in T} C_{a, t} = 1 \\
\label{sch-c-6}
&\forall a \in A, & &\:\textstyle\sum\limits_{\scriptscriptstyle t \in T} S_{a, t} = 1 \\
\label{sch-c-7}
&\forall t \in T, \forall a \in A, & &\:\forall b \in in(a), \:C_{a, t} \leq P(b, t) + R(b, t)\\
\label{sch-c-8}
&\forall t \in T, \forall a \in A, & &\:\forall b \in sib(a), \:C(a, t) = C(b, t)\\
\label{sch-c-9}
&\forall t \in T, & &\:\textstyle\sum\limits_{\scriptscriptstyle a \in A} C_{a, t} = 1
\end{align}
\end{subequations}

==> floats/nas-result-all.tex <==
\begin{figure}[h]
    \centering
    
    % Minipage for the table
    \begin{minipage}[t]{\textwidth}
        \begin{table}[h]
            \captionsetup{font=small}
            \caption{Time-to-solution (in seconds) for the complex NAS DNNs. The left two columns are the solving time for \name with different fixed operator orderings (\S\ref{subsec:ext-fix-order}), and the rightmost column is \name with divide-and-conquer (DnC) heuristic. HMCOS provides operator orderings with minimum peak memory footprint.}
            \setlength\tabcolsep{4pt}
            \centering
            \label{tab:tts-nas-model}
            \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
            \toprule
            \multirow{2}{*}{DNN} & \multicolumn{3}{c|}{Default+COSMA}      & \multicolumn{3}{c|}{HMCOS+COSMA} & \multicolumn{3}{c}{COSMA DnC} \\
                        & $M_R$   & $M_{H}$   & $M_{P}$   & $M_{R}$   & $M_{H}$   & $M_{P}$   & $M_{R}$   & $M_{H}$   & $M_{P}$    \\ \midrule
            PNASNet-5   & 12.2 & 12.3 & 12.2 & 24.2 & 22.4 & 23.5 & 65.9 & 63.5 & 58.0  \\
            AmoebaNet-D & 8.1  & 8.3  & 8.1  & 84.4 & 8.2  & 8.5  & 62.1 & 59.9 & 112.8 \\
            NASNet-A    & 19.8 & 20.0 & 19.7 & 22.4 & 22.4 & 21.6 & 37.5 & 22.9 & 39.2  \\
            DARTS       & 5.0  & 5.0  & 5.0  & 5.2  & 5.2  & 5.2  & 19.1 & 19.1 & 19.1  \\ \bottomrule
            \end{tabular}
            \begin{tablenotes}
                \item $\ast$ Measured on an Apple laptop with M1Pro CPU.
            \end{tablenotes}
        \end{table}
    \end{minipage}
    
    % \vspace{1cm}  % Adjust the vertical spacing as needed
    
    % Minipage for the figure
    \begin{minipage}[t]{\textwidth}
        \begin{figure}[h]
            \centering
            \includegraphics[width=0.48\textwidth]{figs/bft-nas-1col.pdf}
            % \includegraphics[width=0.48\textwidth]{figs/bft-nas-1col-2x2.pdf}
            \captionsetup{font=small}
            \caption{compulsory off-chip data access amount for different solutions on the NAS DNNs. All DNNs take an input tensor of size $(1, 3, 224, 224)$ with 8-bit datatype.}
            \label{fig:data-mov-comp-nas}
        \end{figure}
    \end{minipage}
    
\end{figure}

==> floats/tts-table-reg.tex <==
\begin{table}[h]
\captionsetup{font=small}
\caption{Time-to-solution for \name on ten different DNNs}
% \setlength\tabcolsep{4pt}
\centering
\label{tab:tts-table}
\begin{tabular}{@{}l|rlrlrl@{}}
\toprule
\multirow{2}{*}{DNN} & \multicolumn{6}{c}{Time-to-solution (second)}                                           \\
            & \multicolumn{2}{c}{$M_{require}$} & \multicolumn{2}{c}{$M_{peak}$} & \multicolumn{2}{c}{$M_{(require + peak)/2}$} \\ \midrule
ResNet-50            & 0.032 & \multicolumn{1}{l|}{0.046} & 0.032 & \multicolumn{1}{l|}{0.043} & 0.032 & 0.045 \\
DenseNet             & 0.599 & \multicolumn{1}{l|}{0.747} & 0.514 & \multicolumn{1}{l|}{0.951} & 0.972 & 0.981 \\
ResNeXt              & 0.048 & \multicolumn{1}{l|}{0.057} & 0.043 & \multicolumn{1}{l|}{0.056} & 0.046 & 0.056 \\
R2Plus1D             & 0.038 & \multicolumn{1}{l|}{0.042} & 0.037 & \multicolumn{1}{l|}{0.046} & 0.036 & 0.042 \\
S3D                  & 0.630 & \multicolumn{1}{l|}{0.759} & 0.614 & \multicolumn{1}{l|}{0.760} & 0.616 & 0.761 \\
FCN                  & 0.154 & \multicolumn{1}{l|}{0.138} & 0.136 & \multicolumn{1}{l|}{0.151} & 0.154 & 0.137 \\
LRASPP               & 0.229 & \multicolumn{1}{l|}{0.226} & 0.180 & \multicolumn{1}{l|}{0.197} & 0.215 & 0.231 \\
DeepLabV3   & 0.100 & \multicolumn{1}{l|}{6.964} & 0.093   & \multicolumn{1}{l|}{0.123}  & 0.100        & 17.242       \\
Transformer & 0.140 & \multicolumn{1}{l|}{0.233} & 0.096   & \multicolumn{1}{l|}{0.174}  & 0.092        & 0.224        \\
ViT                  & 0.025 & \multicolumn{1}{l|}{0.020} & 0.017 & \multicolumn{1}{l|}{0.023} & 0.015 & 0.020 \\ \bottomrule
\end{tabular}
\begin{tablenotes}
    \item $\ast$ All experiments run on an Apple laptop with M1Pro CPU.
\end{tablenotes}
\end{table}


% \begin{table*}[t]
% \caption{}
% \label{tab:my-table}
% \setlength\tabcolsep{3pt}
% \begin{tabular}{l|cccccccccccccccccccc}
% \hline
% Mem. Limit &
%   \multicolumn{2}{c}{ResNet-50} &
%   \multicolumn{2}{c}{DenseNet} &
%   \multicolumn{2}{c}{ResNeXt} &
%   \multicolumn{2}{c}{R2Plus1D} &
%   \multicolumn{2}{c}{S3D} &
%   \multicolumn{2}{c}{FCN} &
%   \multicolumn{2}{c}{LRASPP} &
%   \multicolumn{2}{c}{DeepLabV3} &
%   \multicolumn{2}{c}{Transformer} &
%   \multicolumn{2}{c}{ViT} \\ \hline
% Min. MR &
%   0.032 & 0.046 &
%   0.599 & 0.747 &
%   0.048 & 0.057 &
%   0.038 & 0.042 &
%   0.630 & 0.759 &
%   0.154 & 0.138 &
%   0.229 & 0.226 &
%   0.100 & 6.964 &
%   0.140 & 0.233 &
%   0.025 & 0.020 \\
% Min. PMF &
%   0.032 & 0.043 &
%   0.514 & 0.951 &
%   0.043 & 0.056 &
%   0.037 & 0.046 &
%   0.614 & 0.760 &
%   0.136 & 0.151 &
%   0.180 & 0.197 &
%   0.093 & 0.123 &
%   0.096 & 0.174 &
%   0.017 & 0.023 \\
% Half MM &
%   0.032 & 0.045 &
%   0.972 & 0.981 &
%   0.046 & 0.056 &
%   0.036 & 0.042 &
%   0.616 & 0.761 &
%   0.154 & 0.137 &
%   0.215 & 0.231 &
%   0.100 & 17.242 &
%   0.092 & 0.224 &
%   0.015 & 0.020 \\ \hline
% \end{tabular}
% \end{table*}

==> floats/work-comp-tab-2col.tex <==
\begin{table*}[tbp]
\caption{}
\label{tab:work-comp}
\begin{tabular}{@{}lllll@{}}
\toprule
 &
  \multicolumn{1}{c}{Operator Scheduling} &
  \multicolumn{1}{c}{Memory Allocation} &
  \multicolumn{1}{c}{Tensor Replacement} &
  \multicolumn{1}{c}{Other} \\ \midrule
\begin{tabular}[c]{@{}l@{}}PyTorch,\\ TensorFlow\end{tabular} &
  User-defined/Data Dependency &
  \begin{tabular}[c]{@{}l@{}}Dynamic Allocation/\\ Heuristics / User Defined\end{tabular} &
  Heuristics &
  \begin{tabular}[c]{@{}l@{}}Limited support for accelerators,\\ Heavy manual effort\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}Serenity,\\ HMCOS\end{tabular} &
  Min. Peak Memory Footprint &
  N/A, Eval on Heuristics &
  N/A, Eval with Belady &
  \begin{tabular}[c]{@{}l@{}}No memory allocation\\ and tensor replacement.\\ No parameter tensors\end{tabular} \\
MODeL &
  \begin{tabular}[c]{@{}l@{}}ILP-based optimization to\\ minimize memory usage\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}ILP-based optimization to \\ minimize memory usage\end{tabular} &
  N/A &
  \begin{tabular}[c]{@{}l@{}}No replacement and memory\\ allocation solution if spilling occurs\\ Do not scale to complex models\end{tabular} \\
Our Work &
  \begin{tabular}[c]{@{}l@{}}ILP-based optimization to\\ minimizing data access\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}ILP-based optimization with\\ exact solution\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}ILP-based optimization\\ for data access\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Divide-and-Conquer technique to\\ scale up to complex models\end{tabular} \\ \bottomrule
\end{tabular}
\end{table*}
